MTraining: Distributed Dynamic Sparse Attention for Efficient Ultra-Long Context Training

The adoption of long context windows has become a standard feature in Large Language Models (LLMs), as extended contexts significantly enhance their capacity for complex reasoning and broaden their applicability across diverse scenarios. Dynamic sparse attention is a promising approach for reducing the computational cost of long-context. However, efficiently training LLMs with dynamic sparse attention on ultra-long contexts-especially in distributed settings-remains a significant challenge, due in large part to worker- and step-level imbalance. This paper introduces MTraining, a novel distributed methodology leveraging dynamic sparse attention to enable efficient training for LLMs with ultra-long contexts. Specifically, MTraining integrates three key components: a dynamic sparse training pattern, balanced sparse ring attention, and hierarchical sparse ring attention. These components are designed to synergistically address the computational imbalance and communication overheads inherent in dynamic sparse attention mechanisms during the training of models with extensive context lengths. We demonstrate the efficacy of MTraining by training Qwen2.5-3B, successfully expanding its context window from 32K to 512K tokens on a cluster of 32 A100 GPUs. Our evaluations on a comprehensive suite of downstream tasks, including RULER, PG-19, InfiniteBench, and Needle In A Haystack, reveal that MTraining achieves up to a 6x higher training throughput while preserving model accuracy. Our code is available at https://github.com/microsoft/MInference/tree/main/MTraining.

==> sections/abstract.tex <==
\begin{abstract}

The adoption of long context windows has become a standard feature in Large Language Models (LLMs), as extended contexts significantly enhance their capacity for complex reasoning and broaden their applicability across diverse scenarios.
Dynamic sparse attention is a promising approach for reducing the computational cost of long-context training.
However, efficiently training LLMs with dynamic sparse attention on ultra-long contexts, especially in distributed settings, remains a significant challenge, due in large part to worker- and step-level imbalance. This paper introduces MTraining, a novel distributed methodology leveraging dynamic sparse attention to enable efficient training for LLMs with ultra-long contexts. Specifically, MTraining integrates three key components: a distributed sparse index approximating, balanced sparse ring attention, and hierarchical sparse ring attention. These components are designed to synergistically address the computational imbalance and communication overheads inherent in dynamic sparse attention mechanisms during the training of models with extensive context lengths. We demonstrate the efficacy of MTraining by training Qwen2.5-3B and Llama-3.1-8B, successfully expanding its context window from 32K/128K to 512K tokens on a cluster of 32$\times$ A100 GPUs. Our evaluations on a comprehensive suite of downstream tasks, including RULER, PG-19, InfiniteBench, and Needle In A Haystack, reveal that MTraining achieves up to a 6x higher training throughput while preserving model accuracy.

\end{abstract}

==> tabs/latency_breakdown.tex <==
\begin{table}[H]
    % \vspace{-10pt}
    \caption{Latency breakdown of the Forward and Backward pass within a single time of Attention computation in MTraining.}
    \centering
    \small
    \setlength{\tabcolsep}{6pt}
    \renewcommand{\arraystretch}{1.1}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l l c}
        \toprule
        \textbf{Category} & \textbf{Component} & \textbf{Time (ms)} \\
        \midrule
        {\textbf{Forward}}
            & Indexing                          & 1.13 \\
            & Attention Computation for a chunk & 0.51 \\
            & CPU operations                    & 2.08 \\
            & Intra-node KV transmission        & 0.13 \\
            & Inter-node KV transmission        & 0.98 \\
        \midrule
        {\textbf{Backward}} 
            & Backward for all vertical lines             & 1.86 \\
            & Attention Computation for a chunk & 2.65 \\
            & CPU operations                    & 1.90 \\
            & Intra-node KV \& dKV transmission & 0.42 \\
            & Inter-node KV \& dKV transmission & 3.40 \\
        % \midrule
        % {\textbf{Naive Sparse Ring Attention}} 
        %     & Forward Total                     & $1.13 + 2.08 + \mathbf{0.98 \times 31} + 0.51 = 34.10$ \\
        %     & Backward Total                    & $1.86 + 1.90 + \mathbf{3.40 \times 31} + 2.65 = 111.81$ \\
        % \midrule
        % {\textbf{Hierarchical Sparse Ring Attention}} 
        %     & Forward Total                     & $1.13 + 2.08 + \mathbf{0.51 \times 32} = 19.53$ \\
        %     & Backward Total                    & $1.86 + 1.90 + \mathbf{2.65 \times 32} = 88.56$ \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:attn_lat_breakdown}
    % \vspace{-10pt}
\end{table}
